Structured Prediction with Partial Labelling through the Infimum Loss

Annotating datasets is one of the main costs in nowadays supervised learning. The goal of weak supervision is to enable models to learn using only forms of labelling which are cheaper to collect, as partial labelling. This is a type of incomplete annotation where, for each datapoint, supervision is cast as a set of labels containing the real one. The problem of supervised learning with partial labelling has been studied for specific instances such as classification, multi-label, ranking or segmentation, but a general framework is still missing. This paper provides a unified framework based on structured prediction and on the concept of infimum loss to deal with partial labelling over a wide family of learning problems and loss functions. The framework leads naturally to explicit algorithms that can be easily implemented and for which proved statistical consistency and learning rates. Experiments confirm the superiority of the proposed approach over commonly used baselines.

==> infimum loss/core.tex <==
\begin{abstract}
  Annotating datasets is one of the main costs in nowadays supervised learning.
  The goal of weak supervision is to enable models to learn using only forms of
  labelling which are cheaper to collect, as partial labelling. This is a type of
  incomplete annotation where, for each datapoint, supervision is cast as a set
  of labels containing the real one.  The problem of supervised learning with
  partial labelling has been studied for specific instances such as
  classification, multi-label, ranking or segmentation, but a general framework
  is still missing. This paper provides a unified framework based on structured
  prediction and on the concept of {\em infimum loss} to deal with partial
  labelling over a wide family of learning problems and loss functions. The
  framework leads naturally to explicit algorithms that can be easily
  implemented and for which proved statistical consistency and learning rates.
  Experiments confirm the superiority of the proposed approach over commonly
  used baselines. 
\end{abstract}

\section{Introduction}

Fully supervised learning demands tight supervision of large amounts of data, a
supervision that can be quite costly to acquire and constrains the scope of
applications. To overcome this bottleneck, the machine learning community is
seeking to incorporate weaker sources of information in the learning framework.
In this paper, we address those limitations through partial labelling: {\em
  e.g.}, giving only partial ordering when learning user preferences over items,
or providing the label ``flower" for a picture of Arum Lilies\footnote{\small
  \url{https://en.wikipedia.org/wiki/Arum}}, instead of spending a consequent
amount of time to find the exact taxonomy. 

Partial labelling has been studied in the context of
classification~\cite{Cour2011,Nguyen2008}, multilabelling~\cite{Yu2014},
ranking~\cite{Hullermeier2008,Korba2018}, as well as
segmentation~\cite{Verbeek2007,Papandreou2015}, or natural language processing
tasks~\cite{AddedforReviewer1,AddedforReviewer2}, however a generic framework is
still missing. Such a framework is a crucial step towards understanding how to
learn from weaker sources of information, and widening the spectrum of machine
learning beyond rigid applications of supervised learning. Some interesting
directions are provided by~\citet{CidSueiro2014,vanRooyen2018}, to recover the
information lost in a corrupt acquisition of labels. Yet, they assume that the
corruption process is known, which is a strong requirement that we want to relax.

In this paper, we make the following contributions: 
\begin{itemize}
  \item We provide a principled framework to solve the problem of learning with
    partial labelling, via {\em structured prediction}. This approach naturally
    leads to a variational framework built on the {\em infimum loss}. 
  \item We prove that the proposed framework is able to recover the original
    solution of the supervised learning problem under identifiability
    assumptions on the labelling process.  
  \item We derive an explicit algorithm which is easy to train and with strong
    theoretical guarantees. In particular, we prove that it is consistent and we
    provide generalization error rates. 
  \item Finally, we test our method against some simple baselines, on synthetic
    and real examples. We show that for certain partial labelling scenarios with
    symmetries, our infimum loss performs similarly to a simple baseline.
    However in scenarios where the acquisition process of the labels is more
    adversarial in nature, the proposed algorithm performs consistently better. 
\end{itemize}

\section{Partial labelling with infimum loss}\label{sec:partial-labelling}
In this section, we introduce a statistical framework for partial labelling, and
we show that it is characterized naturally in terms of risk minimization with
the infimum loss.  First, let's recall some elements of fully supervised and
weakly supervised learning.

{\em Fully supervised learning} consists in learning a function~${f\in\Y^\X}$
between a input space~$\X$ and a output space~$\Y$, given a joint distribution
${\rho \in \Prob{\X \times \Y}}$ on~${\X \times \Y}$, and a loss function ${\ell
  \in \R^{\Y\times\Y}}$, that minimizes the risk
\begin{equation}\label{eq:risk}
  {\cal R}(f; \rho) = \E_{(X, Y)\sim\rho}\bracket{\ell(f(X), Y)},
\end{equation}
given observations ${(x_i, y_i)_{i\leq n} \sim \rho^{\otimes n}}$. We will
assume that the loss~$\ell$ is proper, {\em i.e.} it is continuous non-negative
and is zero on, and only on, the diagonal of~${\Y \times \Y}$, and strictly
positive outside. We will also assume that $\Y$ is compact.

In \emph{weakly supervised learning},  given~$(x_i)_{i\leq n}$, one does not
have direct observations of~$(y_i)_{i\leq n}$ but weaker information.
The goal is still to recover the solution~${f \in \Y^\X}$ of the fully
supervised problem~\cref{eq:risk}.
In \emph{partial labelling}, also known as \emph{superset learning} or as
\emph{learning with ambiguous labels}, which is an instance of weak supervision,
information is cast as closed sets $(S_i)_{i\leq n}$ in ${\cal S}$, where ${\cal
S}\subset 2^\Y$ is the space of closed subsets of $\Y$, containing the true
labels ${(y_i \in S_i)}$. In this paper, we model this scenario by considering a
data distribution ${\tau \in \Prob{\X \times {\cal S}}}$, that generates the
samples $(x_i, S_i)$. We will denote $\tau$ as {\em weak distribution} to
distinguish it from $\rho$. Capturing the dependence on the original problem,
$\tau$~must be compatible with $\rho$, a matching property that we formalize
with the concept of eligibility. 
%
\begin{definition}[Eligibility]\label{def:eligibility}
  Given a probability measure $\tau$ on $\X \times  {\cal S}$, a probability
  measure $\rho$ on $\X \times \Y$ is said to be eligible for $\tau$ (denoted by
  $\rho \vdash \tau$), if there exists a probability measure $\pi$ over $\X
  \times \Y \times {\cal S}$ such that $\rho$ is the marginal of $\pi$ over $\X
  \times \Y$, $\tau$ is the marginal of $\pi$ over $\X \times  {\cal S}$, and,
  for $y\in\Y$ and $S\in{\cal S}$
  \[
    y\notin S \qquad \Rightarrow \qquad \PP_{\pi}\paren{S\midvert
      Y=y} = 0.
  \]
  We will alternatively say that $\tau$ is a {\em weakening} of~$\rho$, or that
  $\rho$ and $\tau$ are {\em compatible}.
\end{definition}
%
\subsection{Disambiguation principle}\label{sec:disambiguation-principle}

According to the setting described above, the problem of partial labelling is
completely defined by a loss and a weak distribution~$(\ell, \tau)$.
The goal is to recover the solution of the original supervised learning problem
in~\cref{eq:risk} assuming that the original distribution verifies
$\rho\vdash\tau$. Since more than one $\rho$ may be eligible for $\tau$, we
would like to introduce a guiding principle to identify a $\rho^\star$ among
them. With this goal we define the concept of {\em non-ambiguity} for $\tau$,
a setting in which a natural choice for $\rho^\star$ appears.
%
\begin{definition}[Non-ambiguity]\label{def:non-ambiguity}
  For any $x \in \X$, denote by $\tau\vert_x$ the conditional probability of
  $\tau$ given $x$, and define the set $S_x$ as 
    \[ S_x = \bigcap_{S \in \supp(\tau\vert_x)} S. \]
  The weak distribution $\tau$ is said {\em non-ambiguous} if, for every
  $x\in\X$, $S_x$ is a singleton.
  Moreover, we say that $\tau$ is {\em strictly non-ambiguous} if
  it is non-ambiguous and there exists ${\eta\in (0,1)}$ such that,
  for all ${x \in \X}$ and ${z \notin S_x}$
    \[\PP_{S \sim \tau\vert_x}(z \in S) \leq 1 - \eta.\]
\end{definition}
%
This concept is similar to the one by~\citet{Cour2011}, but more subtle because
this quantity only depends on~$\tau$, and makes no assumption on the original
distribution~$\rho$ describing the fully supervised process that we can not
access. In this sense, it is also more general.

When $\tau$ is non-ambiguous, we can write $S_x = \brace{y_x}$ for any $x$,
where $y_x$ is the only element of $S_x$. 
In this case it is natural to identify $\rho^\star$ as the one satisfying
$\rho^\star\vert_x = \delta_{y_x}$. 
Actually, such a $\rho^\star$ is characterized without $S_x$ as the only
deterministic distribution that is eligible for $\tau$. Because deterministic
distributions are characterized as minimizing the minimum risk of~\cref{eq:risk},
we introduce the following {\em minimum variability principle} to disambiguate
between all eligible $\rho$'s, and identify $\rho^\star$,
%
\begin{equation}\label{eq:infimum-disambiguation}
  \rho^\star \in \argmin_{\rho\vdash \tau}{\cal E}(\rho),\qquad
  {\cal E}(\rho) = \inf_{f:\X\to\Y} {\cal R}(f; \rho).
\end{equation}
%
The quantity ${\cal E}$ can be identified as a variance, since if $f_\rho$ is the
minimizer of ${\cal R}(f; \rho)$, $f_\rho(x)$ can be seen as the
mean of $\rho\vert_x$ and $\ell$ the natural distance in $\Y$.
Indeed, when $\ell = \ell_2$ is the mean square loss, this is exactly the case.
%
The principle above recovers exactly $\rho^\star\vert_x = \delta_{y_x}$, when $\tau$ is
non-ambiguous, as stated by~\cref{thm:ambiguity}, proven in~\cref{proof:ambiguity}.
%
\begin{proposition}[Non-ambiguity determinism]\label{thm:ambiguity}
  When $\tau$ is non-ambiguous, the solution $\rho^\star$
  of~\cref{eq:infimum-disambiguation} exists and satisfies that, for any $x\in\X$,
  $\rho^\star\vert_x = \delta_{y_x}$, where $y_x$ is the only element of $S_x$.
\end{proposition}
%
\cref{thm:ambiguity} provides a justification for the usage of the minimum variability principle.
Indeed, under non-ambiguity assumption, following this principle will allow us to
build an algorithm that recover the original fully supervised distribution.
Therefore, given samples $(x_i, S_i)$, it is of interest to test if $\tau$ is
non-ambiguous. Such tests should leverage other regularity hypothesis
on $\tau$, which we will not address in this work.

Now, we characterize the minimum variability principle in terms of a variational
optimization problem that we can tackle in \cref{sec:algorithm} via empirical
risk minimization. 

\subsection{Variational formulation via the infimum loss}
Given a partial labelling problem $(\ell, \tau)$, define the solutions based on
the minimum variablity principle as the functions minimizing the recovered risk
% 
\begin{equation}\label{eq:fstar-of-rhostar}
  f^* \in \argmin_{f:\X \to \Y} {\cal R}(f; \rho^\star).
\end{equation}
% 
for $\rho^\star$ a distribution solving \cref{eq:infimum-disambiguation}.
As shown in~\cref{thm:infimum-loss} below, proven in~\cref{proof:infimum-loss},
the proposed disambiguation paradigm naturally leads to a variational framework
involving the {\em infimum loss}.  
%
\begin{theorem}[Infimum loss (\emph{IL})]\label{thm:infimum-loss} 
  The functions $f^*$ defined in \cref{eq:fstar-of-rhostar} are characterized as
    \[ f^* \in \argmin_{f:\X \to \Y} {\cal R}_S(f), \]
  where the risk ${\cal R}_S$ is defined as
  \begin{equation}\label{eq:set-risk}
    {\cal R}_S(f) = \E_{(X,S)\sim\tau}\bracket{L(f(X), S)},
  \end{equation}
  and $L$ is the  {\em infimum loss}
  \begin{equation}\label{eq:infimum-loss}
    L(z, S) = \inf_{y\in S} \ell(z, y).
  \end{equation}
\end{theorem}
%
The infimum loss, also known as the ambiguous loss \citep{Luo2010,Cour2011},
or as the optimistic superset loss \citep{Hullermeier2014},
captures the idea that, when given a set~$S$, this set contains the good label
$y$ but also a lot of bad ones, that should not be taken into account when
retrieving~$f$. In other terms, $f$ should only match the best guess in $S$.
Indeed, if $\ell$ is seen as a distance, $L$ is its natural extension to sets.

\subsection{Recovery of the fully supervised solutions}
In this subsection, we investigate the setting where an original fully
supervised learning problem $\rho_0$ has been weakened due to incomplete
labelling, leading to a weak distribution~$\tau$. The goal here is to understand
under which conditions on $\tau$ and $\ell$ it is possible to recover the
original fully supervised solution based with the infimum loss framework.
Denote $f_0$ the function minimizing ${\cal R}(f;\rho_0)$.
The theorem below, proven in \cref{proof:non-ambiguity}, shows that under
non-ambiguity and deterministic conditions, it is possible to fully recover
the function $f_0$ also from $\tau$.
%
\begin{theorem}[Supervision recovery]\label{thm:non-ambiguity}
  For an instance $(\ell, \rho_0, \tau)$ of the weakened supervised problem,
  if we denote by $f_0$ the minimizer of~\cref{eq:risk}, we have the under the
  conditions that (1)~$\tau$ is not ambiguous (2)~for all $x\in\X$, $S_x =
  \brace{f_0(x)}$; the infimum loss recovers the original fully supervised
  solution, {\em i.e.} the $f^*$ defined in~\cref{eq:fstar-of-rhostar} verifies
  $f^* = f_0$.

  Futhermore, when $\rho_0$ is deterministic and $\tau$ not ambiguous, the
  $\rho^\star$ defined in~\cref{eq:infimum-disambiguation} verifies $\rho^\star
  = \rho_0$.
\end{theorem}
%
At a comprehensive levels, this theorem states that under non-ambiguity of the
partial labelling process, if the labels are a deterministic function of the
inputs, the infimum loss framework make it possible to recover the solution of
the original fully supervised problem while only accessing weak labels. 
In the next subsection, we will investigate which is the relation between the
two problems when dealing with an estimator $f$ of $f^*$.
%
\subsection{Comparison inequality}\label{sec:calibration}
In the following, we want to characterize the error performed by ${\cal
  R}(f;\rho^\star)$ with respect to the error performed by ${\cal R}_S(f)$. This
will be useful since, in the next section, we will provide an estimator for
$f^*$ based on structured prediction, that minimize the risk ${\cal R}_S$.
First, we introduce a measure of discrepancy for the loss function.  
%
\begin{definition}[Discrepancy of the loss $\ell$]
  Given a loss function $\ell$, the {\em discrepancy degree} $\nu$ of $\ell$ is
  defined as 
    \[ \nu = \log\sup_{y, z'\neq z} \frac{\ell(z, y)}{\ell(z, z')}. \]
  $\Y$ will be said discrete for $\ell$ when $\nu < +\infty$, which is always
  the case when $\Y$ is finite. 
\end{definition}
%
Now we are ready to state the comparison inequality that generalizes to
arbitrary losses and output spaces a result on $0-1$ loss on classification from
\citet{Cour2011}. 
%
\begin{proposition}[Comparison inequality]\label{thm:calibration}
  When $\Y$ is discrete and $\tau$ is strictly non-ambiguous for a given $\eta
  \in (0,1)$, then the following holds  
  \begin{equation}\label{eq:calibration-bound}
    {\cal R}(f; \rho^\star) - {\cal R}(f^*;\rho^\star) \leq C({\cal R}_S(f) - {\cal R}_S(f^*)),
  \end{equation}
  for any measurable function $f \in \Y^\X$, where $C$ does not depend on $\tau,
  f$, and is defined as follows and always finite 
    \[ C = \eta^{-1} e^\nu.\]
\end{proposition}
%
When $\rho_0$ is deterministic, since we know from~\cref{thm:non-ambiguity} that
$\rho^\star=\rho_0$, this theorem allows to bound the error made on the original
fully supervised problem with the error measured with the infimum loss on the
weakly supervised one.

Note that the constant presented above is the product of two independent terms,
the first measuring the ambiguity of the weak distribution $\tau$, and the
second measuring a form of discrepancy for the loss. In the appendix, we provide
a more refined bound for $C$, that is $C = C(\ell, \tau)$, that shows a more
elaborated interaction between $\ell$ and $\tau$. This may be interesting in
situations where it is possible to control the labelling process and may suggest
strategies to active partial labelling, with the goal of minimizing the costs of
labelling while preserving the properties presented in this section and reducing
the impact of the constant $C$ in the learning process. An example is provided
in the \cref{discussion:refinement-C}. 

\section{Consistent algorithm for partial labelling}\label{sec:algorithm}
In this section, we provide an algorithmic approach based on structured
prediction to solve the weak supervised learning problem expressed in terms of
infimum loss from~\cref{thm:infimum-loss}. From this viewpoint, we could
consider different structured prediction frameworks as structured
SVM \cite{Tsochantaridis2005}, conditional random fields \cite{Lafferty2001} or
surrogate mean estimation \cite{Ciliberto2016}. For example, \citet{Luo2010}
used a margin maximization formulation in a structured SVM fashion,
\citet{Hullermeier2015} went for nearest neighbors,
and \citet{Cour2011} design a surrogate method specific to the 0-1 loss, for
which they show consistency based on~\citet{Bartlett2006}. 

In the following, we will use the structured prediction method
of~\citet{Ciliberto2016,Nowak2019}, which allows us to derive an explicit
estimator, easy to train and with strong theoretical properties, in particular,
consistency and finite sample bounds for the generalization error.
The estimator is based on the pointwise characterization of $f^*$ as
\[
  f^*(x) \in \argmin_{z\in\Y} \E_{S\sim \tau\vert_x}\bracket{\inf_{y\in S}\ell(z, y)},
\]
and weights $\alpha_i(x)$ that are trained on the dataset such that
$\hat{\tau}_{\vert x} = \sum_{i=1}^n \alpha_i(x) \delta_{S_i}$ is a good
approximation of $\tau\vert_x$.
Plugging this approximation in the precedent equation leads to our estimator,
that is defined explicity as follows
%
\begin{equation}\label{eq:algorithm}
  f_n(x) \in \argmin_{z\in\Y} \inf_{y_i \in S_i} \sum_{i=1}^n \alpha_i(x) \ell(z, y_i).
\end{equation}
%
Among possible choices for $\alpha$, we will consider the following kernel ridge
regression estimator to be learned at training time
\[
  \alpha(x) = (K + n\lambda)^{-1}v(x),
\]
with $\lambda > 0$ a regularizer parameter and $K = (k(x_i, x_j))_{i,j} \in
\R^{n\times n}, v(x) = (k(x, x_i))_{i} \in \R^n$ where $k\in \X\times\X \to \R$
is a positive-definite kernel \cite{Scholkopf2001} that defines a similarity
function between input points  ({\em e.g.}, if $\X = \R^d$ for some $d \in \N$ a
commonly used kernel is the Gaussian kernel $k(x,x') = e^{-\|x-x'\|^2}$). Other
choices can be done to learn $\alpha$, beyond kernel methods, a particularly
appealing one is harmonic functions, incorporating a prior on low density
separation to boost learning \cite{Zhu2003,Zhou2003,Bengio2006}. Here we use the
kernel estimator since it allows to derive strong theoretical results, based on
kernel conditional mean estimation \cite{Muandet2017}.

\subsection{Theoretical guarantees}
In this following, we want to prove that $f_n$ converges to $f^*$ as
$n$ goes to infinity and we want to quantify it with finite sample bounds. The
intuition behind this result is that as the number of data points tends toward
infinity, $\hat{\tau}$ concentrates towards $\tau$, making our algorithm in
\cref{eq:algorithm} converging to a minimizer of~\cref{eq:set-risk} as explained
more in detail in \cref{proof:consistency}.
%
\begin{theorem}[Consistency]\label{thm:consistency}
  Let $\Y$ be finite and $\tau$ be a non-ambiguous probability. Let $k$ be a
  bounded continuous universal kernel, {\em e.g.} the Gaussian kernel
  \citep[see][for details]{Micchelli2006}, and $f_n$ the estimator in
  \cref{eq:algorithm} trained on $n \in \N$ examples and with $\lambda =
  n^{-1/2}$. Then, holds with probability~$1$ 
    \[ \lim_{n \to \infty} {\cal R}(f_n; \rho^\star) = {\cal R}(f^*; \rho^\star).\]
\end{theorem}
%
In the next theorem, instead we want to quantify how fast $f_n$ converges to
$f^*$ depending on the number of examples. To obtain this result, we need a
finer characterization of the infimum loss $L$ as: 
\[
  L(z, S) = \scap{\psi(z)}{\phi(S)},
\]
where ${\cal H}$ is a Hilbert space and $\psi: \Y \to {\cal H}, \phi: 2^{\Y} \to
{\cal H}$ are suitable maps. Such a decomposition always exists in finite case (as
for the infimum loss over $\Y$ finite) and many explicit examples for losses of
interest are presented by~\citet{Nowak2019}. We now introduce the conditional
expectation of $\phi(S)$ given $x$, defined as 
\function{g}{\X}{\cal H}{x}{\E_{\tau}\bracket{\phi(S)\midvert X = x}.}
The idea behind the proof is that the distance between $f_n$ and $f$ is bounded
by the distance of $g_n$ an estimator of $g$ that is implicitly computed via
$\alpha$. If $g$ has some form of regularity, {\em e.g.} $g \in {\cal
  G}$, with ${\cal G}$ the space of functions representable by the chosen kernel
\citep[see][]{Scholkopf2001}, then it is possible to derive explicit rates, as
stated in the following theorem. 
%
\begin{theorem}[Convergence rates]\label{thm:learning-rates}
  In the setting of~\cref{thm:consistency}, if $\tau$ is $\eta$-strictly non
  ambiguous for $\eta\in(0, 1)$, and if $g \in {\cal G}$, then there exists a
  $\tilde{C}$, such that, for any $\delta \in (0, 1)$ and $n\in \N$, holds with
  probability at least $1 - \delta$,
  \begin{equation}\label{eq:rates}
    {\cal R}(f_n; \rho^\star) - {\cal R}(f^*; \rho^\star) \leq
    \tilde{C} \log\paren{\frac{8}{\delta}}^2 n^{-1/4}.
  \end{equation}
\end{theorem}
%
Those last two theorem are proven in \cref{proof:consistency} and combines the
consistency and learning results for  kernel ridge regression
\cite{Caponnetto2007,Smale2007}, with a comparison inequality
of~\citet{Ciliberto2016} which relates the excess risk of the structured
prediction problem with the one of the surrogate loss ${\cal R}_S$, together
with our \cref{thm:calibration}, which relates the error ${\cal R}$ to ${\cal
  R}_S$. 

Thoses results make our algorithm the first algorithm for partial labelling,
that to our knowledge is applicable to a generic loss $\ell$ and has strong
theoretical guarantees as consistency and learning rates. In the next section we
will compare with the state of the art and other variational principles. 

\section{Previous works and baselines}
\label{sec:inconsistency}
Partial labelling was first approached through discriminative models, proposing to
learn $\paren{Y \midvert X}$ among a family of parameterized distributions
% by $\theta \in \Theta$
by maximizing the log likelihood
  % \[ \Lcal((x_i, S_i)_{i\leq n}; \theta) = \sum_{i=1}^n\log
  % \paren{\sum_{y\in S_i}\PP\paren{y\midvert x_i; \theta}},\]
based on expectation-maximization scheme~\cite{Jin2002}, eventually integrating
knowledge on the partial labelling process~\cite{Grandvalet2002,Papandreou2015}.
In the meanwhile, some applications of clustering methods have involved special
instances of partial labelling, like segmentation approached with spectral
method~\cite{Weiss1999}, semi-supervision approached with
max-margin~\cite{Xu2004}. 
Also initially geared towards clustering,~\citet{Bach2007} consider the infimum
principle on the mean square loss, and this was generalized to weakly supervised
problems~\cite{Joulin2010}. 
The infimum loss as an objective to minimize when learning from partial labels
was introduced by~\citet{Cour2011} for the classification instance and used
by~\citet{Luo2010,Hullermeier2014} in generic cases. 
Comparing to those last two, we provide a
framework that derives the use of infimum loss from first principles and from
which we derive an explicit and easy to train algorithm with strong statistical
guarantees, which were missing in previous work.
In the rest of the section, we will compare the infimum loss with other
variational principles that have been considered in the literature, in
particular the supremum loss~\cite{Guillaume2017} and the average loss~\cite{Denoeux2013}. 

\paragraph{Average loss (\emph{AC}).}
A simple loss to deal with uncertainty is to average over all potential
candidates, assuming $S$ discrete,
\[
  L_{\textit{ac}}(z, S) = \frac{1}{\module{S}} \sum_{y\in S} \ell(z, y).
\]
It is equivalent to a fully supervised distribution $\rho_{\textit{ac}}$ by
sampling $Y$ uniformly at random among $S$ 
  \[ \rho_{\textit{ac}}(y) = \int_{{\cal S}} \frac{1}{\module{S}} \ind{y\in S} \diff\tau(S).\]
This directly follows from the definition of $L_{\textit{ac}}$ and of the risk
${\cal R}(z; \rho_{\textit{ac}})$. However, as soon as the loss $\ell$ has
discrepancy, {\em i.e.} $\nu > 0$, the average loss will implicitly advantage
some labels, which can lead to inconsistency, even in the deterministic not
ambiguous setting of~\cref{thm:calibration} (see \cref{app:other-losses} for
more details).

\paragraph{Supremum loss (\emph{SP}).}
Another loss that have been considered is the supremum
loss~\cite{Wald1945,Madry2018}, bounding from above the fully supervised risk
in~\cref{eq:risk}. It is widely used in the context of robust risk minimization
and reads
\[
  R_{\textit{sp}}(f) = \sup_{\rho\vdash\tau} \E_{(X,Y)\sim\rho}\bracket{\ell(f(x), S)}.
\]
Similarly to the infimum loss in~\cref{thm:infimum-loss}, this risk can be
written from the loss function
\[
  L_{\textit{sp}}(z, S) = \sup_{y\in S} \ell(z, y).
\]
Yet, this adversarial approach is not consistent for partial labelling, even in
the deterministic non ambiguous setting of~\cref{thm:calibration}, since it
finds the solution that best agrees with {\em all} the elements in $S$ and not
only the true one (see \cref{app:other-losses} for more details).

\subsection{Instance showcasing superiority of our method}
In the rest of this section, we consider a pointwise example to showcase the
underlying dynamics of the different methods.
It is illustrated in~\cref{fig:inconsistency}.
%
Consider $\Y = \brace{a, b, c}$ and a proper symmetric loss function such that
$\ell(a, b) = \ell(a, c) = 1$, $\ell(b, c) = 2$. 
The simplex $\Prob{\Y}$ is naturally split into decision regions, for $e\in\Y$,
\[
  R_e = \brace{\rho\in\Prob{\Y} \midvert e\in\argmin_{z\in\Y}\E_{\rho}[\ell(z, Y)]}.
\]
Both {\em IL} and {\em AC} solutions can be understood geometrically by looking
at where $\rho^\star$ and $\rho_{\textit{ac}}$ fall in the partition of the
simplex $(R_e)_{e\in\Y}$. Consider a fully supervised problem with distribution
$\delta_c$, and a weakening $\tau$ of $\rho$ defined by
$\tau(\brace{a, b, c}) = \frac{5}{8}$ and
$\tau(\brace{c}) = \tau(\brace{a,c}) = \tau(\brace{b,c}) = \frac{1}{8}$.
This distribution can be represented on the simplex  in terms of the region
$R_\tau = \brace{\rho\in\Prob{\Y}\midvert \rho\vdash \tau}$. 
Finding $\rho^\star$ correspond to minimizing the piecewise linear function $
{\cal E}(\rho)$~(\cref{eq:infimum-disambiguation}) inside $R_\tau$. On this
example, it is minimized for $\rho^\star = \delta_c$, which we know from
~\cref{thm:calibration}. Now note that if we use the average loss, it
disambiguates $\rho$ as 
\[
  \rho_{\textit{ac}}(c) = \frac{11}{24} =
  \frac{1}{3}\frac{5}{8} + \frac{1}{8} + 2\cdot\frac{1}{2}\frac{1}{8}, \quad
  \rho_{\textit{ac}}(b) = \rho_{\textit{ac}}(a) = \frac{13}{48}.
\]
This distribution falls in the decision region of $a$, which is inconsistent
with the real label $y=c$. 
For the supremum loss, one can show, based on ${\cal R}_{\textit{sp}}(a) = \ell(a, c) =
1$, ${\cal R}_{\textit{sp}}(b) = \ell(b, c) = 2$ and ${\cal R}_{\textit{sp}}(c) =
3/2$, that the supremum loss is minimized for $z = a$, which is also
inconsistent. Instead, by using the infimum loss, we have $f^* = f_0 = c$, and
moreover that $\rho^\star = \rho_0$ that is the optimal one.
%
\begin{figure}[h]
  \centering
  \input{drawings/inconsistency}
  \vspace*{-.3cm}  
  \caption{Simplex $\Prob{\Y}$. (Left) Decision frontiers. (Middle left) Full
    and weak distributions. (Middle right) Level curves of the piecewise linear
    objective ${\cal E}$~(\cref{eq:infimum-disambiguation}), to optimize when
    disambiguating $\tau$ into $\rho^\star$. (Right) Disambiguation of
    \emph{AC}  and \emph{IL}.}
\label{fig:inconsistency}
\end{figure}
%
\subsection{Algorithmic considerations for AC, SP}
The averaging candidates principle, approached with the framework of quadratic
surrogates \cite{Ciliberto2016}, leads to the following algorithm
%
\begin{align*}
  f_{\textit{ac}}(x) &\in \argmin_{z\in\Y}
      \sum_{i=1}^n \alpha_{i}(x)\frac{1}{\module{S_i}}\sum_{y\in S_i} \ell(z, y)
   \\ &= \argmin_{z\in\Y} \sum_{y\in\Y}
      \paren{\sum_{i=1}^n \mathbf{1}_{y\in S_i}\frac{\alpha_i(x)}{ \module{S_i}}} \ell(z,y).
\end{align*}
%
This estimator is computationally attractive because the inference complexity is
the same as the inference complexity of the original problem when approached with the
same structured prediction estimator. Therefore, one can directly reuse
algorithms developed to solve the original inference problem~\cite{Nowak2019}.
Finally, with a similar approach to the one in \cref{sec:algorithm}, we can
derive the following algorithm for the supremum loss
\[
  f_{\textit{sp}}(x) \in \argmin_{z\in\Y}
      \sup_{y_i \in S_i}\sum_{i=1}^n \alpha_i(x) \ell(z, y_i).
\]
In the next section, we will use the average candidates as baseline to compare
with the algorithm proposed in this paper, as the supremum loss consistently
performs worth, as it is not fitted for partial labelling.

\section{Applications and experiments}\label{sec:application}
In this section, we will apply \cref{eq:algorithm} to some synthetic and real
datasets from different prediction problems and compared with the average
estimator presented in the section above, used as a baseline. Code is available
online.\footnote{\url{https://github.com/VivienCabannes/partial_labelling}}

\subsection{Classification}\label{sec:classification}
Classification consists in recognizing the most relevant item among $m$ items.
The output space is isomorphic to the set of indices $\Y=\bbracket{1, m}$, and
the usual loss function is the 0-1 loss 
\[
  \ell(z, y) = \ind{y\neq z}. 
\]
It has already been widely studied with several approaches that are calibrated
in non ambiguous deterministic setting, notably by~\citet{Cour2011}. The infimum
loss reads $L(z, S) = \ind{z\notin S}$, and its risk in~\cref{eq:set-risk} is
minimized for 
\[
  f(x) \in \argmax_{z\in \Y} \PP\paren{z\in S \midvert X=x}.
\]
Based on data $(x_i, S_i)_{i\leq n}$, our estimator~\cref{eq:algorithm} reads
\[
  f_n(x) = \argmax_{z\in\Y} \sum_{i;z\in S_i} \alpha_i(x).
\]
For this instance, the supremum loss is really conservative, only learning from
set that are singletons $L_{\textit{sp}}(z, S) = \ind{S\neq\brace{z}}$, while the
average loss is similar to the infimum one, adding an evidence weight depending
on the size of $S$, $L_{\textit{ac}}(z, S) \simeq \ind{z\notin S} / \module{S}$. 
%
\begin{figure}[h]
  \centering
  \includegraphics{images/cl/dna.pdf}
  \vspace* {-.3cm}
  \includegraphics{images/cl/svmguide2.pdf}
  \vspace*{-.3cm}  
  \caption{Classification. Testing risks (from~\cref{eq:risk}) achieved by {\em
      AC} and {\em IL} on the ``dna'' and ``svmguide2'' datasets from {\em
      LIBSVM} as a function of corruption parameter $c$, when the corruption is
    as follows: for $y$ being the most present labels of the dataset, and
    $z'\neq z$,  $\PP\paren{z'\in S\midvert Y=z} = c\cdot \ind{z=y}$. Plotted
    intervals show the standard deviation on eight-fold cross-validation.
    Experiments were done with the Gaussian kernel. See all experimental details
    in~\cref{app:experiments}.}
  \label{fig:libsvm}
\end{figure}
%
\paragraph{Real data experiment.} To compare {\em IL} and {\em AC}, we used {\em
  LIBSVM} datasets~\cite{Chang2011} on which we corrupted labels to simulate
partial labelling. When the corruption is uniform, the two methods perform the
same. Yet, when labels are unbalanced, such as in the ``dna'' and ``svmguide2''
datasets, and we only corrupt the most frequent label $y\in\Y$, the infimum loss
performs better as shown in~\cref{fig:libsvm}. 

\subsection{Ranking}\label{sec:ranking}
Ranking consists in ordering $m$ items based on an input~$x$ that is often the
conjunction of a user $u$ and a query $q$, ($x=(u,q)$). An ordering can be
thought as a permutation, that is, $\Y=\Sfrak_m$. While designing a loss for
ranking is intrinsincally linked to a voting system \cite{Arrow1950}, making it
a fundamentally hard problem; \citet{Kemeny1959} suggested to approach it
through pairwise disagreement, which is current machine learning
standard~\cite{Duchi2010}, leading to the Kendall embedding 
\[
  \phi(y) = \paren{\sign\paren{y_i - y_j}}_{i<j \leq m},
\]
and the Kendall loss~\citep{Kendall1938}, with $C = m(m-1)/2$
\[
    \ell(y, z) = C - \phi(y)^T\phi(z). 
\]
Supervision often comes as partial order on items, {\em e.g.},
\[
  S = \brace{y\in\Sfrak_m \midvert y_i > y_j > y_k, y_l > y_m}.
\]
It corresponds to fixing some coordinates in the Kendall embedding. In this
setting, \emph{AC} and \emph{SP} are not consistent, as one can recreate a
similar situation to the one in~\cref{sec:inconsistency}, considering $m=3$, $a
= (1,2,3)$, $b=(2,1,3)$ and $c=(1,3,2)$ (permutations being represented with
$(\sigma^{-1}(i))_{i\leq m}$), and supervision being most often $S = (1>3) =
\brace{a,b,c}$ and sometimes $S = (1>3>2) = \brace{c}$.

\paragraph{Minimum feedback arc set.}
Dealing with Kendall's loss requires to solve problem of the form,
\[
 \argmin_{y \in S} \scap{c}{\phi(y)},
\]
for $c\in\R^{m^2}$, and constraints due to partial ordering encoded in
$S\subset\Y$. This problem is an instance of the constrained minimum feedback
arc set problem.We provide a simple heuristic to solve it in~\cref{app:fas},
which consists of approaching it as an integer linear program. Such heuristics
are analyzed and refined for analysis purposes
by~\citet{Ailon2005,vanZuylen2007}.

\paragraph{Algorithm specification.}
At inference, the infimum loss requires to solve:
\begin{equation}\tag{\ref{eq:algorithm}}
  f_n(x) = \argmax_{z\in\Y} \sup_{(y_i) \in S_i} \sum_{i=1}^n \alpha_i(x) \scap{\phi(z)}{\phi(y_i)}.
\end{equation}
It can be approached with alternate minimization, initializing $\phi(y_i) \in
\hull(\phi(S_i))$, by putting $0$ on unseen observed pairwise comparisons, then,
iteratively, solving a minimum feedback arc set problem in $z$, then solving
several minimum feedback arc set problems with the same objective, but different
constraints in $(y_i)$. This is done efficiently using warmstart on the dual
simplex algorithm. 
% 
\begin{figure}[h]
  \centering
  \includegraphics{images/rk/setting.pdf}
  \vspace*{-.3cm}
  \caption{Ranking, experimental setting. Colors represent four different items
    to rank. Each item is associate to a utility function of $x$ shown on the
    left figure. From those scores, is retrieved an ordering $y$ of the items as
    represented on the right.}
  \label{fig:rk:setting}
\end{figure}
% 
\begin{figure}[h]
  \centering
  \includegraphics{images/rk/corruption.pdf}
  \vspace* {-.3cm}
  \caption{Ranking, results. Testing risks~(from \cref{eq:risk}) achieved by
    {\em AC} and {\em IL} as a function of corruption parameter $c$. When $c=1$,
    both risks are similar at $0.5$. The simulation setting is the same as
    in~\cref{fig:libsvm}. The error bars are defined as for~\cref{fig:libsvm},
    after cross-validation over eight folds. {\em IL} clearly outperforms {\em
      AC}.} 
  \label{fig:rk:corruption}
\end{figure}

\begin{figure*}[t]
  \centering
  \includegraphics{images/ir/setting.pdf}
  \vspace* {-.3cm}
  \includegraphics{images/ir/reconstruction.pdf}
  \vspace* {-.3cm}
  \caption{Partial regression on $\R$. In this setting we aim at recovering a
    signal $y(x)$ given upper and lower bounds on it amplitude, and in thirty
    percent of case, information on its phase, or equivalently in $\R$, its
    sign. {\em IL} clearly outperforms the baseline. Indeed {\em AC} is a
    particular ill-fitted method on such a problem, since it regresses on the
    barycenters of the resulting sets.} 
  \label{fig:interval-regression}
\end{figure*}

\paragraph{Synthetic experiments.}
Let us consider $\X = [0,1]$ embodying some input features. Let $\{1,\dots,m\}$,
$m \in \N$ be abstract items to order, each item being linked to a utility
function $v_i \in \R^\X$, that characterizes the value of $i$ for $x$ as
$v_i(x)$. Labels $y(x)\in\Y$ are retrieved by sorting $(v_i(x))_{i\leq m}$.
To simulate a problem instance, we set $v_i$ as $v_i(x) = a_i\cdot x + b_i$,
where $a_i$ and $b_i$ follow a standard normal distribution. Such a setting is
illustrated in~\cref{fig:rk:setting}. 

After sampling $x$ uniformly on $[0, 1]$ and retrieving the ordering $y$ based
on scores, we simulate partial labelling by randomly loosing pairwise
comparisons. The comparisons are formally defined as coordinates of the
Kendall's embedding $(\phi(y)_{jk})_{jk\leq m}$. To create non symmetric
perturbations we corrupt more often items whose scores differ a lot. In other
words, we suppose that the partial labelling focuses on pairs that are hard to
discriminate. The corruption is set upon a parameter $c\in[0,1]$. In fact, for
$m=10$, until $c=0.5$, our corruption is fruitless since it can most often be
inverted based on transitivity constraint in ordering, while the problem becomes
non-trivial with $c \geq 0.5$.  In the latter setting, {\em IL} clearly
outperforms {\em AC} on~\cref{fig:rk:corruption}. 

\subsection{Partial regression}\label{sec:partial-regression}
Partial regression is an example of non discrete partial labelling problem,
where $\Y=\R^m$ and the usual loss is the Euclidean distance 
\[
 \ell(y, z) = \norm{y - z}^2.
\]
This partial labelling problem consists of regression where observation are sets
$S\subset \R^m$ that contains the true output $y$ instead that $y$. Among
others, it arises for example in economical models, where bounds are preferred
over approximation when acquiring training labels~\cite{Tobin1958}.
%
As an example, we will illustrate how partial regression could appear for
some phase problems arising with physical measurements.
Suppose a physicist want to measure the law between a vectorial
quantity $Y$ and some input parameters~$X$. Suppose that, while she can record the
input parameters $x$, her sensors do not exactly measure $y$ but render an
interval in which the amplitude $\norm{y}$ lays and only occasionally render
its phase $y / \norm{y}$, in a fashion that leads to a set of candidates $S$ for
$y$. The geometry over $\ell^2$ makes it a perfect example to showcase
superiority of the infimum loss as illustrated in~\cref{fig:interval-regression}.

In this figure, we consider ${\cal Y} = \mathbb{R}$ and suppose that $Y$ is a
deterministic function of $X$ as shown by the dotted blue line signal.  If,
for a given $x_i$, measurements only provides that $\module{y_i} \in [1, 2]$
without the sign of $y_i$, a situation where the phase is lost, this
correspond to the set $S_i = [-2, -1] \cup [1, 2]$, explaining the shape of
observed sets that are symmetric around the origin.
Whenever the acquired data has no phase, which happen seventy percent of the
time in our simulation, AC will target the set centers, explaining the green
curve. On the other hand, IL is aiming at passing by each set, which
explains the orange curve, crossing all blue bars.

\section{Conclusions}
In this paper, we deal with the problem of weakly supervised learning, beyond
standard regression and classification, focusing on the more general case of
arbitrary loss functions and structured prediction. We provide a principled
framework to solve the problem of learning with partial labelling, from which a
natural variational approach based on the infimum loss is derived. We prove that
under some identifiability assumptions on the labelling process the framework is
able to recover the solution of the original supervised learning problem. The
resulting algorithm is easy to train and with strong theoretical guarantees. 
In particular we prove that it is consistent and we provide generalization error
rates. Finally the algorithm is tested on simulated and real datasets, showing
that when the acquisition process of the labels is more adversarial in nature,
the proposed algorithm performs consistently better than baselines. This paper
focuses on the problem of partial labelling, however the resulting mathematical
framework is quite flexible in nature and it is  interesting to explore the
possibility to extend it to tackle also other weakly supervised problems, as
imprecise labels from non-experts~\cite{Dawid1979}, more general constraints
over the set $(y_i)_{i\leq n}$ \cite{Quadrianto2009} or semi-supervision
\cite{Chapelle2006}.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% reftex-default-bibliography: ("main.bib")
%%% End:


==> infimum loss/drawings/consistency.tex <==
\begin{tikzpicture}[scale=3]
  \coordinate(a) at (0, 0);
  \coordinate(b) at ({cos(60)}, {sin(60)});
  \coordinate(c) at (1, 0);
  \coordinate(r) at ({1/4}, 0);
  \coordinate(s) at ({7/32 + 1/8}, {7*sin(60)/16});
  \coordinate(t) at ({3/8 + 1/4}, {3*sin(60)/4});

  \coordinate(ra) at ({1/4},0);
  \coordinate(rb) at ({3/8},{-sin(60)/4});
  \coordinate(rc) at ({5/8},{-sin(60)/4});
  \coordinate(rd) at (1,{sin(60)/2});
  \coordinate(re) at ({1/2},{sin(60)/2});
  
  \fill[fill=black!10] (c) -- (r) -- (s) -- (t) -- cycle;
  % \fill[fill=black!10] (a) -- (r) -- (s) -- (t) -- (b) -- cycle;
  \fill[fill=black!30] (ra) -- (rb) -- (rc) -- (rd) -- (re) -- cycle;
  \draw (a) node[anchor=north east]{a} -- (b) node[anchor=south]{b} -- (c) node[anchor=south west]{c} -- cycle;
  \draw (c) -- (r) -- (s) -- (t) -- cycle;
  \draw (ra) -- (rb) -- (rc) -- (rd) -- (re) -- cycle;
  \node at ({5/8}, {sin(60)/2 + 1/16}) {$R_{\tau}$};
  \node at ({9/16}, {-sin(60)/4 + 1/8}) {$R_{\hat{\tau}}$};
  \fill[fill=red!100] (1, 0) circle (.1em) node[anchor=north west] {$\rho^\star$};
  \fill[fill=red!100] ({5/8}, {-sin(60)/4}) circle (.1em) node[anchor=north west] {$\hat\rho$};

  \foreach \x in {0,.05,...,.6}
  \draw[gray, very thin, rotate=30] (1.25, \x) -- ({sin(60) - (tan(60)*\x)}, \x) -- ({sin(60) - (tan(60)*\x)}, -\x) -- ({1.25}, {-\x}); 

  \draw[dashed, rotate=30] (1.25, 0) -- ({sin(60)}, 0) -- ({sin(60) - (tan(60)*.55)}, .55); 
  \draw[dashed, rotate=30] ({sin(60)}, 0) --  ({sin(60) - (tan(60)*.55)}, -.55); 
\end{tikzpicture}

==> infimum loss/drawings/inconsistency.tex <==
\begin{tikzpicture}[scale=2.5]
  \coordinate(a) at (0, 0);
  \coordinate(b) at ({1/2}, {sin(60)});
  \coordinate(c) at (1, 0);
  \coordinate(ha) at ({3/4}, {sin(60)/2});
  \coordinate(hb) at ({1/2}, 0);
  \coordinate(hc) at ({1/4}, {sin(60)/2});

  \coordinate (mc) at (1,-.25);
  \coordinate (mca) at (0,-.25);
  \fill[fill=white] (a) -- (c) -- (mc) -- (mca) -- cycle;

  \fill[fill=red!20] (a) -- (hb) -- (ha) -- (hc) -- cycle;
  \fill[fill=green!20] (b) -- (ha) -- (hc) -- cycle;
  \fill[fill=blue!20] (c) -- (ha) -- (hb) -- cycle;
  \draw (a) node[anchor=north east]{a} -- (b) node[anchor=south]{b} --
        (c) node[anchor=north west]{c} -- cycle;
  \draw (hb) -- (ha) -- (hc);
  \node at ({3/8}, {sin(60)/4}) {$R_a$};
  \node at ({1/2}, {3*sin(60)/4 - 1/16}) {$R_b$};
  \node at ({3/4}, {sin(60)/4 - 1/16}) {$R_c$};
\end{tikzpicture}
\begin{tikzpicture}[scale=2.5]
  \coordinate(a) at (0, 0);
  \coordinate(b) at ({cos(60)}, {sin(60)});
  \coordinate(c) at (1, 0);
  \coordinate(r) at ({1/4}, 0);
  \coordinate(s) at ({7/32 + 1/8}, {7*sin(60)/16});
  \coordinate(t) at ({3/8 + 1/4}, {3*sin(60)/4});

  \coordinate (mc) at (1,-.25);
  \coordinate (mca) at (0,-.25);
  \fill[fill=white] (a) -- (c) -- (mc) -- (mca) -- cycle;

  \fill[fill=black!20] (c) -- (r) -- (s) -- (t) -- cycle;
  \fill[fill=black!10] (a) -- (r) -- (s) -- (t) -- (b) -- cycle;
  \draw (a) node[anchor=north east]{a} -- (b) node[anchor=south]{b} --
        (c) node[anchor=south west]{c} -- cycle;
  \draw (c) -- (r) -- (s) -- (t) -- cycle;
  \node at ({5/8}, {sin(60)/3 - 1/16}) {$R_{\tau}$};
  \fill[fill=black!60] (1, 0) circle (.1em) node[anchor=north west] {$\rho_0$};
\end{tikzpicture}
\begin{tikzpicture}[scale=2.5]  
  \coordinate (a) at (0,0) ;
  \coordinate (b) at ({1/2},{sin(60)}) ;
  \coordinate (c) at (1,0);
  \coordinate (mb) at (.25, {sin(60)});
  \coordinate (mba) at ({-.25*cos(30)},{.25*sin(30)});
  \coordinate (mc) at (1,-.25);
  \coordinate (mca) at (0,-.25);
  \coordinate(ha) at ({3/4}, {sin(60)/2});
  \coordinate(hb) at ({1/2}, 0);
  \coordinate(hc) at ({1/4}, {sin(60)/2});

  \foreach \x in {0,.05,...,.25}
  \draw[gray, rotate=30] ({sin(60)}, \x) -- ({sin(60) - (tan(60)*\x)}, \x) --
  ({sin(60) - (tan(60)*\x)}, -\x) -- ({sin(60)}, {-\x}); 
  \foreach \x in {0.25,.3,...,.5}
  \draw[gray, rotate=30] ({sin(60)}, \x) -- ({sin(60)-tan(60)*(.5-\x)}, \x);
  \foreach \x in {0.25,.3,...,.5}
  \draw[gray, rotate=30] ({sin(60)-tan(60)*(.5-\x)}, -\x) -- ({sin(60)}, {-\x}); 
  \foreach \x in {.25,.3,...,.5}
  \draw[gray, rotate=30] ({sin(60) - (tan(60)*\x)}, .25) -- ({sin(60) - (tan(60)*\x)}, -.25); 

  \fill[fill=white] (a) -- (c) -- (mc) -- (mca) -- cycle;
  \fill[fill=white] (a) -- (b) -- (mb) -- (mba) -- cycle;
  \draw (a) node[anchor=north east]{a} -- (b) node[anchor=south]{b} --
  (c) node[anchor=north west]{c} -- cycle;
  \draw[dotted, thick] (hc) -- (ha) -- (hb);
\end{tikzpicture}
\begin{tikzpicture}[scale=2.5]
  \coordinate(a) at (0, 0);
  \coordinate(b) at ({1/2}, {sin(60)});
  \coordinate(c) at (1, 0);
  \coordinate(ha) at ({3/4}, {sin(60)/2});
  \coordinate(hb) at ({1/2}, 0);
  \coordinate(hc) at ({1/4}, {sin(60)/2});
  \coordinate(r) at ({1/4}, 0);
  \coordinate(s) at ({7/32 + 1/8}, {7*sin(60)/16});
  \coordinate(t) at ({3/8 + 1/4}, {3*sin(60)/4});

  \coordinate (mc) at (1,-.25);
  \coordinate (mca) at (0,-.25);
  \fill[fill=white] (a) -- (c) -- (mc) -- (mca) -- cycle;

  \fill[fill=red!20] (a) -- (hb) -- (ha) -- (hc) -- cycle;
  \fill[fill=green!20] (b) -- (ha) -- (hc) -- cycle;
  \fill[fill=blue!20] (c) -- (ha) -- (hb) -- cycle;
  \draw (a) node[anchor=north east]{a} -- (b) node[anchor=south]{b} --
        (c) node[anchor=south west]{c} -- cycle;
  \draw (hb) -- (ha) -- (hc);
  \draw[densely dotted] (c) -- (r) -- (s) -- (t) -- cycle;
  \fill[fill=black!60] (1, 0) circle (.1em) node[anchor=north west] {$\rho^\star$};
  \fill[fill=black!60] ({13/96+11/24}, {13*sin(60)/48}) circle (.1em)
                       node[anchor=south east] {$\rho_{\textit{ac}}$};
\end{tikzpicture}

==> infimum loss/drawings/simplex_calibration.tex <==
\begin{tikzpicture}[scale=3]
  \coordinate(a) at (0, 0);
  \coordinate(b) at ({cos(60)}, {sin(60)});
  \coordinate(c) at (1, 0);
  \coordinate(r) at ({1/4}, 0);
  \coordinate(s) at ({7/32 + 1/8}, {7*sin(60)/16});
  \coordinate(t) at ({3/8 + 1/4}, {3*sin(60)/4});

  \fill[fill=black!20] (c) -- (r) -- (s) -- (t) -- cycle;
  \draw (a) node[anchor=north east]{a} -- (b) node[anchor=south]{b} --
        (c) node[anchor=north west]{c} -- cycle;
  \draw (c) -- (r) -- (s) -- (t) -- cycle;
  \node at ({5/8}, {sin(60)/3 - 1/16}) {$R_{\tau}$};
  \fill[fill=black!60] (1, 0) circle (.075em);

  \foreach \x in {0,.125,...,1} \draw[gray]
           ({\x / 2}, {\x*sin(60)}) -- ({(3 - \x) / 4)}, {(1 + \x) * sin(60)/2}); 
  \foreach \x in {0,.125,...,1} \draw[gray]
           ({\x, 0}) -- ({(3 + \x) / 4)}, {(1 - \x) * sin(60)/2});
  \draw (-.5,0) -- ({7/8}, {11*sin(60)/12});
  \draw (-.5,{sin(60)/3}) node[anchor=east] {$\delta_b + D_b$} -- ({3/4}, {7*sin(60)/6});
  \draw[<->] ({3/4}, {5*sin(60)/6}) -- ({11/16}, {23*sin(60)/24}) node[anchor=south west]
             {$\quad \frac{1}{4}\, d(b, c) \propto {\cal R}_S(b) =
              {\cal R}(b; \frac{1}{4}\delta_c + \frac{3}{4}\delta_b)$} -- ({5/8}, {13*sin(60)/12});    
  \draw[<->] ({1/2 + 3 * .04 / 2}, {(1 + .04) * sin(60)})  --
             ({7/8}, {2*(1 + 2*.04 - 7/8)*sin(60)}) node[anchor=south west]
             {$\, d(b, c) \propto {\cal R}(b; \delta_c)$} -- ({1 + 3 * .04 / 2}, {.04*sin(60)});    
\end{tikzpicture}

==> infimum loss/drawings/thales.tex <==
\begin{tikzpicture}[scale=1]
  \coordinate(xz1) at (0,3);
  \coordinate(xz2) at (7,3);
  \coordinate(xs1) at (0,2);
  \coordinate(xs2) at (7,2);
  \coordinate(xy1) at (0,0);
  \coordinate(xy2) at (7,0);
  \coordinate(s1) at (2,0);
  \coordinate(s2) at (4,0);
  \coordinate(s3) at (4,1);
  \coordinate(s4) at (3,2);
  \coordinate(s5) at (1,.5);
  \draw (xz1) node[anchor=east] {$z + x^\perp$} -- (xz2);
  \draw (xs1) node[anchor=east] {\footnotesize{$\lambda y + (1-\lambda)z + x^\perp$}} -- (xs2);
  \draw (xy1) node[anchor=east] {$y + x^\perp$} -- (xy2);
  \filldraw[fill=black!20] (s1) -- (s2) -- (s3) -- (s4) -- (s5) -- cycle;

  \fill[fill=black] (2,0) circle (.2em) node[anchor=north west] {$y$};
  \fill[fill=black] (1,3) circle (.2em) node[anchor=north west] {$z$};

  \coordinate(d1) at (4.5,2);
  \coordinate(d2) at (4.5,2.5);
  \coordinate(d3) at (4.5,3);
  \draw[<->, dashed] (d1) -- (d2) node [anchor=west] {\footnotesize{$\,\,\,\lambda d(z+x^\perp, y)$}} -- (d3);
  \coordinate(s) at (3, 1);
  \draw (s) node [anchor=north] {$S$};
\end{tikzpicture}

==> infimum loss/template/macro.tex <==
% Non mathematic commands
\newcommand{\quot}[1]{``#1''}
\newcommand\note[1]{\textcolor{red}{#1}}
% \renewcommand\note[1]{}

%% Symboles
% ... math usual operators
\newcommand{\diff}{\mathop{}\!\mathrm{d}}
\DeclareMathOperator{\E}{\mathbb{E}}
\DeclareMathOperator{\PP}{\mathbb{P}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator{\mean}{mean}
\DeclareMathOperator{\var}{var}

% ... less usual operators
\newcommand{\Prob}[1]{\Delta_{#1}}
\newcommand{\ind}[1]{\mathbf{1}_{#1}}
\newcommand{\simiid}{\sim_{\scriptscriptstyle{iid.}}}
\newcommand{\uniform}[1]{\mathcal{U}\paren{#1}}
\DeclareMathOperator{\Span}{Span}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\hull}{Conv}
\DeclareMathOperator{\ima}{Im}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator*{\supp}{supp}
\DeclareMathOperator{\trace}{Tr}
% \DeclareMathOperator{\cov}{cov}
% \DeclareMathOperator{\Div}{div}
% \DeclareMathOperator{\grad}{grad}
% \DeclareMathOperator{\spec}{spec}

% ... math usual variables
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}

% ... brackets
\newcommand{\bangle}[1]{\left\langle #1 \right\rangle}
\newcommand{\bbracket}[1]{\left\llbracket #1 \right\rrbracket}
\renewcommand{\brace}[1]{\left\{ #1 \right\}}
\newcommand{\bracket}[1]{\left[ #1 \right]}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\paren}[1]{\left( #1 \right)}
\newcommand{\midvert}{\,\middle\vert\,}

% ... brackets type operations
\newcommand{\module}[1]{\left| #1 \right|}
\newcommand{\norm}[1]{\left\| #1 \right\|}
\newcommand{\scap}[2]{\left\langle #1, #2 \right\rangle}

% ... abbreviation
\newcommand{\Sfrak}{\mathfrak{S}}

%% Specific
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}

%% Command
\newcommand{\deriv}[2]{\frac{\mathrm d #1}{\mathrm d #2}}

% ... aethestic
\renewcommand{\epsilon}{\varepsilon}
\renewcommand{\phi}{\varphi}

% % ... missing symbols
\newcommand{\independent}{\protect\mathpalette{\protect\independenT}{\perp}}
\def\independenT#1#2{\mathrel{\rlap{$#1#2$}\mkern2mu{#1#2}}}


%% Environments
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
% \theoremstyle{definition}
\newtheorem{definition}{Definition}
%\theoremstyle{remark}
\newtheorem*{remark}{Remark}



% Optimization problems
\newcommand{\minimize}[2]{
\[
\begin{array}{rl}
	\text{minimize } & #1 \\
	\text{subject to } & #2 
\end{array}
\]
}

% Function
\newcommand{\function}[5]{
\[
\begin{array}{cccc}
	#1 : & #2 & \rightarrow & #3 \\
	 & #4 & \rightarrow & #5
\end{array}
\]
}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% reftex-default-bibliography: ("main.bib")
%%% End:

==> infimum loss/template/package.tex <==
% Packages
\usepackage[english]{babel}
\usepackage[T1]{fontenc}
\usepackage[utf8]{inputenc}

% Formatting
\usepackage{enumitem}
\usepackage{microtype}

% Graphics
\usepackage{graphicx}
% \usepackage{subfigure}
\usepackage{caption}
\usepackage{tikz}
\usepackage{booktabs}
\usepackage{blkarray}

% Coloring
\usepackage{xcolor}

% Math packages
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{stmaryrd}
\usepackage{amsthm}

% Algorithmique packages
% \usepackage{algorithm}
% \usepackage{algpseudocode}
\newcommand{\theHalgorithm}{\arabic{algorithm}}

% Boxing equations
\usepackage{empheq}

% Links
\PassOptionsToPackage{hyphens}{url}
\usepackage{hyperref}
\usepackage{url}
\usepackage{cleveref}
\usepackage{natbib}

% Several Bibliographies
\usepackage{multibib}
\newcites{appendix}{Appendix References}

% Itemize
\setitemize{
	itemsep=0pt, 
	label={--},
    parsep=0pt, 
    topsep=0pt
}

\setenumerate{
	itemsep=0pt,
    parsep=0pt, 
    topsep=0pt
}

% Cleverref
\crefname{section}{Sec.}{Secs.}
\crefname{appendix}{Appendix}{Appendices}
\crefname{equation}{Eq.}{Eqs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{table}{Tab.}{Tabs.}

\crefname{theorem}{Thm.}{Thms.}
\crefname{proposition}{Prop.}{Props.}
\crefname{corollary}{Cor.}{Cors.}
\crefname{lemma}{Lem.}{Lems.}
\crefname{definition}{Def.}{Defs.}
\crefname{remark}{Rmk.}{Rmks.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% reftex-default-bibliography: ("main.bib")
%%% End:
